Does HD 3167 Have Planets with Perpendicular Orbits?

The two transiting planets of HD 3167 were reported to follow nearly perpendicular paths, with the inner orbit aligned with the stellar equator and the outer orbit nearly polar. This interpretation depends critically on a challenging single-transit detection of the Rossiter-McLaughlin effect of the inner planet. We observed three additional transits of the inner planet with the Keck Planet Finder and analyzed the new data together with two archival ESPRESSO transit datasets. We do not confirm the previously reported low obliquity. Our analysis favors a projected obliquity of $-66^{+14}_{-12}$ degrees, consistent with coplanar orbits. However, because the best-fit projected rotation velocity is higher than expected, and because the obliquity uncertainty grows substantially when the most discrepant of the five transit datasets is omitted, we regard the geometry of the HD 3167 system as still unsettled.

==> rv_kpf_espresso.tex <==
\begin{deluxetable}{@{}rccc@{}}
\tablecaption{Relative RV measurements of HD\,3167.
\label{tbl:rv_kpf_espresso}}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{BJD} &
\colhead{RV\,(m/s)} &
\colhead{$\sigma_{\rm RV}$\,(m/s)} &
\colhead{Instrument}
}
\startdata
2460209.87884 & 1.685 & 0.531 & KPF \\
2460209.88286 & 2.633 & 0.566 & KPF \\
2460209.88699 & 2.049 & 0.577 & KPF \\
2460209.89096 & 3.174 & 0.793 & KPF \\
2460209.89519 & 2.564 & 0.646 & KPF \\
2460209.89904 & 2.871 & 0.584 & KPF \\
2460209.90309 & 2.915 & 0.585 & KPF \\
2460209.90705 & 2.147 & 0.582 & KPF \\
2460209.91123 & 1.938 & 0.556 & KPF \\
2460209.91519 & 1.690 & 0.566 & KPF \\
2460209.91925 & 2.761 & 0.551 & KPF \\
2460209.92333 & 1.655 & 0.537 & KPF \\
2460209.92726 & 1.597 & 0.567 & KPF \\
2460209.94723 & 0.738 & 0.553 & KPF \\
2460209.95174 & 0.085 & 0.548 & KPF \\
2460209.95858 & 0.981 & 0.531 & KPF \\
2460209.96229 & 1.878 & 0.546 & KPF \\
2460209.96637 & 1.298 & 0.608 & KPF \\
2460209.97051 & 1.251 & 0.537 & KPF \\
2460209.97452 & 1.768 & 0.532 & KPF \\
2460209.97859 & 1.404 & 0.527 & KPF \\
2460209.98258 & 0.354 & 0.527 & KPF \\
2460209.98665 & 0.708 & 0.538 & KPF \\
2460209.99062 & -0.136 & 0.557 & KPF \\
2460209.99476 & -0.109 & 0.544 & KPF \\
2460209.99870 & 1.033 & 0.547 & KPF \\
2460210.00257 & -0.801 & 0.595 & KPF \\
2460210.00681 & 0.859 & 0.666 & KPF \\
2460210.01081 & -0.145 & 0.617 & KPF \\
2460210.01468 & 0.672 & 0.666 & KPF \\
2460210.01875 & -0.716 & 0.752 & KPF \\
2460210.02303 & -0.494 & 0.673 & KPF \\
2460210.02709 & -1.639 & 0.701 & KPF \\
2460210.03103 & -1.478 & 0.626 & KPF \\
2460210.03492 & -0.775 & 0.685 & KPF \\
2460210.03913 & -0.598 & 0.749 & KPF \\
2460210.04332 & -0.434 & 0.790 & KPF \\
2460210.04704 & -1.288 & 0.698 & KPF \\
2460210.05122 & -1.192 & 0.823 & KPF \\
2460210.05520 & 0.190 & 0.722 & KPF \\
2460210.05928 & -0.197 & 0.825 & KPF \\
2460210.06342 & -1.122 & 0.764 & KPF \\
2460210.06711 & -1.185 & 0.821 & KPF \\
2460210.07203 & -2.712 & 0.986 & KPF \\
2460210.07524 & -1.226 & 0.824 & KPF \\
2460210.08163 & -2.411 & 0.645 & KPF \\
2460210.08543 & -2.819 & 0.668 & KPF \\
2460210.08970 & -3.715 & 0.570 & KPF \\
2460210.09331 & -2.024 & 0.644 & KPF \\
2460210.09743 & -2.702 & 0.856 & KPF \\
2460210.85419 & 2.047 & 0.543 & KPF \\
2460210.85823 & 2.838 & 0.545 & KPF \\
2460210.86214 & 1.661 & 0.550 & KPF \\
2460210.86639 & 1.595 & 0.557 & KPF \\
2460210.87024 & 2.211 & 0.558 & KPF \\
2460210.87433 & 1.845 & 0.583 & KPF \\
2460210.87839 & 1.699 & 0.562 & KPF \\
2460210.88233 & 2.311 & 0.566 & KPF \\
2460210.88639 & 2.310 & 0.568 & KPF \\
2460210.89056 & 1.696 & 0.570 & KPF \\
2460210.89455 & 1.755 & 0.606 & KPF \\
2460210.89853 & 1.147 & 0.646 & KPF \\
2460210.90256 & 1.775 & 0.614 & KPF \\
2460210.90686 & 1.358 & 0.604 & KPF \\
2460210.91079 & 2.389 & 0.558 & KPF \\
2460210.91463 & 1.635 & 0.548 & KPF \\
2460210.91875 & 1.144 & 0.573 & KPF \\
2460210.92278 & 0.643 & 0.576 & KPF \\
2460210.92681 & 1.225 & 0.545 & KPF \\
2460210.93084 & 1.311 & 0.524 & KPF \\
2460210.93484 & 1.221 & 0.560 & KPF \\
2460210.93901 & 1.603 & 0.624 & KPF \\
2460210.94297 & 0.923 & 0.575 & KPF \\
2460210.94693 & 0.925 & 0.567 & KPF \\
2460210.95102 & 1.638 & 0.569 & KPF \\
2460210.95508 & 0.762 & 0.568 & KPF \\
2460210.95904 & 0.943 & 0.600 & KPF \\
2460210.96313 & 0.524 & 0.569 & KPF \\
2460210.96721 & -0.742 & 0.553 & KPF \\
2460210.97121 & 0.400 & 0.555 & KPF \\
2460210.97523 & 0.268 & 0.539 & KPF \\
2460210.97930 & -0.881 & 0.523 & KPF \\
2460210.98330 & -0.186 & 0.549 & KPF \\
2460210.98738 & -1.017 & 0.581 & KPF \\
2460210.99138 & -1.596 & 0.547 & KPF \\
2460210.99543 & -0.913 & 0.547 & KPF \\
2460210.99939 & -1.789 & 0.584 & KPF \\
2460211.00354 & -1.131 & 0.570 & KPF \\
2460211.00760 & -1.490 & 0.558 & KPF \\
2460211.01155 & -1.754 & 0.525 & KPF \\
2460211.01559 & -1.337 & 0.541 & KPF \\
2460211.01966 & -1.379 & 0.539 & KPF \\
2460211.02375 & -1.752 & 0.553 & KPF \\
2460211.02774 & -2.156 & 0.567 & KPF \\
2460211.03178 & -2.705 & 0.540 & KPF \\
2460211.03581 & -2.469 & 0.533 & KPF \\
2460211.03983 & -2.446 & 0.532 & KPF \\
2460211.04394 & -2.055 & 0.536 & KPF \\
2460211.04790 & -3.598 & 0.527 & KPF \\
2460211.05209 & -2.486 & 0.514 & KPF \\
2460211.05605 & -2.539 & 0.538 & KPF \\
2460211.06019 & -2.516 & 0.518 & KPF \\
2460211.06408 & -3.682 & 0.535 & KPF \\
2460237.74671 & 0.833 & 0.711 & KPF \\
2460237.75058 & 2.117 & 0.662 & KPF \\
2460237.75476 & 1.058 & 0.642 & KPF \\
2460237.75874 & 1.738 & 0.617 & KPF \\
2460237.76278 & 1.015 & 0.695 & KPF \\
2460237.76681 & 1.206 & 0.668 & KPF \\
2460237.77082 & 0.388 & 0.718 & KPF \\
2460237.77493 & 1.095 & 0.747 & KPF \\
2460237.77891 & 1.995 & 0.685 & KPF \\
2460237.78297 & 1.922 & 0.694 & KPF \\
2460237.78717 & 1.145 & 0.710 & KPF \\
2460237.79099 & 1.431 & 0.615 & KPF \\
2460237.79511 & 1.646 & 0.635 & KPF \\
2460237.79914 & 1.449 & 0.584 & KPF \\
2460237.80314 & 0.493 & 0.596 & KPF \\
2460237.80717 & 0.996 & 0.641 & KPF \\
2460237.81119 & 1.283 & 0.628 & KPF \\
2460237.81529 & -0.222 & 0.659 & KPF \\
2460237.81926 & -0.455 & 0.680 & KPF \\
2460237.82334 & 0.000 & 0.651 & KPF \\
2460237.82740 & 1.034 & 0.610 & KPF \\
2460237.83140 & -0.136 & 0.616 & KPF \\
2460237.83547 & -0.492 & 0.609 & KPF \\
2460237.83977 & -1.352 & 0.597 & KPF \\
2460237.84349 & -0.132 & 0.598 & KPF \\
2460237.84758 & -0.788 & 0.584 & KPF \\
2460237.85156 & 0.354 & 0.593 & KPF \\
2460237.85562 & 0.225 & 0.574 & KPF \\
2460237.85960 & -0.131 & 0.591 & KPF \\
2460237.86366 & -1.106 & 0.579 & KPF \\
2460237.86772 & -0.618 & 0.603 & KPF \\
2460237.87178 & 0.215 & 0.576 & KPF \\
2460237.87575 & -1.653 & 0.569 & KPF \\
2460237.87978 & -0.519 & 0.597 & KPF \\
2460237.88383 & -0.650 & 0.585 & KPF \\
2460237.88788 & -0.929 & 0.609 & KPF \\
2460237.89189 & -0.977 & 0.615 & KPF \\
2460237.89661 & -0.886 & 0.649 & KPF \\
2460237.90062 & -1.159 & 0.669 & KPF \\
2460237.90463 & -2.191 & 0.651 & KPF \\
2460237.90879 & -1.278 & 0.676 & KPF \\
2460237.91277 & -1.766 & 0.665 & KPF \\
2460237.91673 & -1.889 & 0.652 & KPF \\
2460237.92065 & -2.266 & 0.667 & KPF \\
2460237.92542 & -1.566 & 0.693 & KPF \\
2460237.92954 & -2.598 & 0.684 & KPF \\
2460237.93351 & -2.993 & 0.664 & KPF \\
2460237.94162 & -1.849 & 0.630 & KPF \\
2460237.94553 & -2.018 & 0.623 & KPF \\
2460237.95018 & -3.813 & 0.626 & KPF \\
2460237.95390 & -1.842 & 0.632 & KPF \\
2460237.95777 & -2.252 & 0.630 & KPF \\
2460237.96243 & -3.221 & 0.637 & KPF \\
2460237.96584 & -3.580 & 0.635 & KPF \\
2458765.80726 & -2.536 & 0.990 & ESPRESSO \\
2458765.81127 & -2.475 & 1.041 & ESPRESSO \\
2458765.81552 & -1.853 & 1.229 & ESPRESSO \\
2458765.81977 & -0.339 & 1.036 & ESPRESSO \\
2458765.65934 & 0.479 & 0.866 & ESPRESSO \\
2458765.66348 & 2.530 & 0.863 & ESPRESSO \\
2458765.66768 & 1.794 & 0.718 & ESPRESSO \\
2458765.67201 & -0.162 & 0.685 & ESPRESSO \\
2458765.67611 & 1.379 & 0.736 & ESPRESSO \\
2458765.68033 & -0.248 & 0.738 & ESPRESSO \\
2458765.68458 & 0.130 & 0.791 & ESPRESSO \\
2458765.68867 & 0.024 & 0.783 & ESPRESSO \\
2458765.69265 & 0.276 & 0.901 & ESPRESSO \\
2458765.69695 & 1.600 & 0.857 & ESPRESSO \\
2458765.70109 & 0.548 & 0.769 & ESPRESSO \\
2458765.70525 & 1.516 & 0.708 & ESPRESSO \\
2458765.70939 & -1.144 & 0.832 & ESPRESSO \\
2458765.71382 & -0.006 & 0.841 & ESPRESSO \\
2458765.71786 & 1.481 & 0.724 & ESPRESSO \\
2458765.72204 & 1.394 & 0.587 & ESPRESSO \\
2458765.72633 & 0.000 & 0.610 & ESPRESSO \\
2458765.73040 & 0.623 & 0.548 & ESPRESSO \\
2458765.73455 & -0.510 & 0.687 & ESPRESSO \\
2458765.73863 & -1.397 & 0.626 & ESPRESSO \\
2458765.74308 & 0.258 & 0.713 & ESPRESSO \\
2458765.74754 & 0.008 & 0.957 & ESPRESSO \\
2458765.75125 & -0.977 & 0.691 & ESPRESSO \\
2458765.75553 & -0.936 & 0.806 & ESPRESSO \\
2458765.75961 & 0.013 & 0.789 & ESPRESSO \\
2458765.76376 & -1.260 & 0.617 & ESPRESSO \\
2458765.76792 & 0.949 & 0.620 & ESPRESSO \\
2458765.77212 & 1.210 & 0.713 & ESPRESSO \\
2458765.77623 & 0.095 & 0.906 & ESPRESSO \\
2458765.78051 & -0.539 & 0.945 & ESPRESSO \\
2458765.78475 & -0.820 & 0.864 & ESPRESSO \\
2458765.78879 & -1.025 & 0.833 & ESPRESSO \\
2458765.79302 & -1.687 & 0.901 & ESPRESSO \\
2458765.79741 & -0.419 & 1.007 & ESPRESSO \\
2458765.80157 & -0.792 & 0.990 & ESPRESSO \\
2459886.52204 & 0.979 & 0.601 & ESPRESSO \\
2459886.52481 & 1.493 & 0.583 & ESPRESSO \\
2459886.52777 & 1.493 & 0.539 & ESPRESSO \\
2459886.53069 & 1.142 & 0.581 & ESPRESSO \\
2459886.53365 & 2.069 & 0.502 & ESPRESSO \\
2459886.53653 & 1.909 & 0.520 & ESPRESSO \\
2459886.53951 & 1.075 & 0.496 & ESPRESSO \\
2459886.54239 & 1.612 & 0.516 & ESPRESSO \\
2459886.54539 & 1.262 & 0.512 & ESPRESSO \\
2459886.54832 & 0.506 & 0.478 & ESPRESSO \\
2459886.55121 & 1.686 & 0.467 & ESPRESSO \\
2459886.55416 & 0.769 & 0.484 & ESPRESSO \\
2459886.55709 & 0.645 & 0.524 & ESPRESSO \\
2459886.56002 & 1.058 & 0.491 & ESPRESSO \\
2459886.56297 & 1.058 & 0.482 & ESPRESSO \\
2459886.56590 & 0.643 & 0.482 & ESPRESSO \\
2459886.56879 & 1.328 & 0.472 & ESPRESSO \\
2459886.57172 & 1.636 & 0.503 & ESPRESSO \\
2459886.57463 & -0.007 & 0.506 & ESPRESSO \\
2459886.57759 & 0.193 & 0.523 & ESPRESSO \\
2459886.58050 & 1.726 & 0.530 & ESPRESSO \\
2459886.58345 & -0.047 & 0.535 & ESPRESSO \\
2459886.58637 & 0.864 & 0.537 & ESPRESSO \\
2459886.58930 & 0.351 & 0.512 & ESPRESSO \\
2459886.59223 & 0.849 & 0.499 & ESPRESSO \\
2459886.59515 & 0.007 & 0.561 & ESPRESSO \\
2459886.59810 & 0.919 & 0.467 & ESPRESSO \\
2459886.60102 & 1.165 & 0.468 & ESPRESSO \\
2459886.60394 & 1.037 & 0.479 & ESPRESSO \\
2459886.60687 & 0.762 & 0.453 & ESPRESSO \\
2459886.60981 & 0.406 & 0.443 & ESPRESSO \\
2459886.61274 & -0.542 & 0.457 & ESPRESSO \\
2459886.61567 & -1.167 & 0.457 & ESPRESSO \\
2459886.61856 & -0.578 & 0.479 & ESPRESSO \\
2459886.62152 & -0.698 & 0.515 & ESPRESSO \\
2459886.62441 & -0.742 & 0.537 & ESPRESSO \\
2459886.62740 & -0.482 & 0.511 & ESPRESSO \\
2459886.63034 & -1.167 & 0.505 & ESPRESSO \\
2459886.63327 & -0.242 & 0.512 & ESPRESSO \\
2459886.63616 & -1.743 & 0.518 & ESPRESSO \\
2459886.63912 & -1.108 & 0.528 & ESPRESSO \\
2459886.64199 & -0.667 & 0.530 & ESPRESSO \\
2459886.64500 & -1.200 & 0.497 & ESPRESSO \\
2459886.64791 & -0.757 & 0.481 & ESPRESSO \\
2459886.65085 & -0.503 & 0.444 & ESPRESSO \\
2459886.65373 & -1.940 & 0.474 & ESPRESSO \\
2459886.65668 & -1.104 & 0.490 & ESPRESSO \\
2459886.65958 & -2.156 & 0.581 & ESPRESSO \\
2459886.66252 & -1.906 & 0.550 & ESPRESSO \\
2459886.66545 & -0.648 & 0.539 & ESPRESSO \\
2459886.66841 & -0.600 & 0.514 & ESPRESSO \\
2459886.67134 & -1.523 & 0.532 & ESPRESSO \\
2459886.67433 & -1.293 & 0.488 & ESPRESSO \\
2459886.67717 & -1.076 & 0.428 & ESPRESSO \\
2459886.68011 & -1.116 & 0.414 & ESPRESSO \\
2459886.68296 & -1.383 & 0.430 & ESPRESSO \\
2459886.68594 & -0.553 & 0.414 & ESPRESSO \\
2459886.68891 & -2.132 & 0.419 & ESPRESSO \\
\enddata
\end{deluxetable}

